The Cost of Coverage: Conformalising Native Forecast Uncertainty for GB Wind Power

Uncertainty bands on wind forecasts help inform reserve sizing and commitments, but often fail to deliver their stated coverage. We apply conformal prediction to native bands to see what it adds and what it costs, comparing six forecasters, from ARIMA to a tabular foundation model, at two wind farms in Great Britain (GB) under operational conditions. We show that calibration repairs empirical marginal coverage with little or no Winkler Score penalty, but this apparent success conceals under-coverage in high winds. Calibrating by forecast wind regime turns marginal coverage into regime-level coverage, cutting day-ahead out-of-band volume in high winds by over 40% relative to pooled calibration while narrowing bands overall.

==> tables/table_missed_energy_by_band.tex <==
\begin{tabular}{@{}llcccccccccccc@{}}
\toprule
 &  & \multicolumn{3}{c}{Periods} & \multicolumn{3}{c}{MWh} & \multicolumn{3}{c}{Energy share} & \multicolumn{3}{c}{Long share} \\
 &  & Low & Average & High & Low & Average & High & Low & Average & High & Low & Average & High \\
Farm & Method &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{3}{*}{Kelmarsh} & Native & 0.25 & 0.66 & 0.09 & 0.02 & 0.06 & 0.26 & 0.08 & 0.58 & 0.34 & 0.12 & 0.66 & 0.94 \\
 & OSSCP & 0.25 & 0.66 & 0.09 & 0.02 & 0.05 & 0.23 & 0.08 & 0.58 & 0.35 & 0.14 & 0.68 & 0.94 \\
 & Mondrian-OSSCP & 0.25 & 0.66 & 0.09 & 0.02 & 0.05 & 0.13 & 0.08 & 0.69 & 0.23 & 0.20 & 0.66 & 0.90 \\
\cmidrule{1-14}
\multirow[t]{3}{*}{Penmanshiel} & Native & 0.32 & 0.56 & 0.12 & 0.04 & 0.15 & 0.50 & 0.08 & 0.55 & 0.38 & 0.18 & 0.64 & 0.91 \\
 & OSSCP & 0.32 & 0.56 & 0.12 & 0.05 & 0.14 & 0.50 & 0.09 & 0.53 & 0.38 & 0.13 & 0.69 & 0.93 \\
 & Mondrian-OSSCP & 0.32 & 0.56 & 0.12 & 0.07 & 0.14 & 0.29 & 0.18 & 0.58 & 0.25 & 0.09 & 0.70 & 0.92 \\
\cmidrule{1-14}
\bottomrule
\end{tabular}

